Graph Signal Processing: Overview, Challenges and Applications

Research in Graph Signal Processing (GSP) aims to develop tools for processing data defined on irregular graph domains. In this paper we first provide an overview of core ideas in GSP and their connection to conventional digital signal processing. We then summarize recent developments in developing basic GSP tools, including methods for sampling, filtering or graph learning. Next, we review progress in several application areas using GSP, including processing and analysis of sensor network data, biological data, and applications to image processing and machine learning. We finish by providing a brief historical perspective to highlight how concepts recently developed in GSP build on top of prior research in other areas.

==> HistoricalPerspective.tex <==
%\subsection{A historical perspective}% {\red (JM)}}

%Links to existing methods/ideas:
%\begin{itemize}
%\item spectral graph theory,
%\item image segmentation,
%\item Transforms and dictionaries,
%\item algebraic signal processing,
%\item Others?  Graphical models? Probabilistic models? Network analysis?
%\end{itemize}
%With the advent of large \textit{un}structured datasets there has been an explosion of activity in developing new methods to infer knowledge from these data. 
%We will focus our discussion on data whose dependencies (structure) are captured by generic arbitrary graphs. We first consider in Section~\ref{subsubsec:connectionsotherareas} connections to related areas like Network Science, Network Processes, and Graphical Models that also address data structured by graphs but deal with different questions and take a different perspective, and then in Section~\ref{subsubsec:historiacalperspective} overview  prior work that has led more directly to graph signal processing.
%
\subsubsection{Related work in other areas}
\label{subsubsec:connectionsotherareas}
%
With the advent of large \textit{un}structured datasets there has been an explosion of activity in developing new methods to infer knowledge from these data. Next we briefly discuss how problems and methods studied in areas such as 
%In this Section, we distinguish graph signal processing from work in 
network science, network processes, and graphical models, relate to those studied in GSP.  

\textbf{Network Science} addresses issues such as uncovering community relations, perceived alliances, quantifying connectedness, or determining the relevance of specific agents. Thus, much of this work focuses on studying what can be learned from the graphs structuring the data, rather than on the data itself. For example, determining the size of the giant component, distribution of component sizes, degree and clique distributions, clustering coefficients, betweeness and closeness centralities, path length, and network diameter \cite{newman2010networks,jackson2010social,easley2010networks}. In the literature, these questions are often the realm of what many call Network Science \cite{networksciencenas,borner2007network,lewis2011network,barabasi2016network}. Connections between this area of research and GSP primarily come from the fact that the graph spectra that GSP builds upon are strongly related to the structure of the graph \cite{Chung:96}. As an example, spectral clustering methods use the low frequency eigenvectors of the Laplacian and thus can be viewed from a GSP perspective \cite{Tremblay:2016vb}. 
%Loosely speaking, a low pass filter used in GSP will tend to smooth attribute values within a community. 

\textbf{Network processes} aim to model propagation over networks, including such phenomena  
as diffusion of disease and epidemics, spread of (fake) news, memes, fads, voting trends, imitation and social influence, propagation of failures and blackouts.  Common models are similar to stochastic automata where the state of the nodes (the ``data'') evolve through local rules, i.e., according to exogeneous (external to the network) and endogeneous (internal to the network) effects. For example, using terminology from epidemics, nodes of the graph representing agents or individuals of a population can be infected (adopt an opinion or spread a rumor, or a failed component), or susceptible (open to adopt an opinion or spread a rumor, or a performing component). Infected or failed nodes can heal and become susceptible again; susceptible nodes can become infected either by an action external to the network or by action of infected neighbors \cite{castellano2012competing,nowzari2016analysis}. Analysis of these network processes is difficult. Traditionally, the network is abstracted out, assuming that any node can infect any other node (full mixing or complete network).  To account for the impact of the network \cite{ganesh2005effect}, resorting to numerical studies is precluded except for very small networks since the network state space $\{0,1\}^N$ grows exponentially fast ($2^N$, for $N$ agents). To study these processes \cite{butts2009revisiting,colizza2006role} one usually considers one of two asymptotic regimes:
%\begin{itemize}
\begin{inparaenum}[1)]
\item either long term behavior (time-asymptotics) and attempting to find the equilibrium distribution of the process \cite{zhang2014diffusion,zhang2015role}; or
\item large network asymptotics (mean field approximation) \cite{draief2010epidemics} leading to the study of the qualitative behavior of nonlinear ordinary differential equations \cite{santos2015bi}.
%\end{itemize}
\end{inparaenum}
Because asymptotic behavior can be seen to depend on the eigenstructure of the underlying graph, GSP representations as those discussed in Section~\ref{sec:representations} can be used to characterize the evolution of a system. As an example, several papers have explored the use of GSP techniques to improve the efficiency of value function estimation in a reinforcement learning scenario \cite{levorato2012structure,levorato2012reduced}. 
%\textbf{Graphical models.} 

In the machine learning and statistics literature, there has been a concerted effort on \textbf{graphical models} focusing on inference and learning from large datasets, \cite{lauritzen1996graphical,jordan1998learning,wainwright2008graphical,koller2009probabilistic,whittaker2009graphical}. The data is modeled as a set of random variables described by a family of Gibbs probability distributions, and the underlying graph, whose nodes label the variables, captures statistical dependence and conditional independence among the data. Acyclic graphs \cite{bang2008digraphs,edwards2012introduction} represent Bayesian networks, while undirected graphs represent Markov random fields \cite{rozanov1982markov,kindermann1980markov,rue2005gaussian}. Graphical models exploit factorizations of the joint distribution to develop efficient message passing algorithms for inference and they find application in many areas, including in modeling texture and other features in image processing \cite{besag1974spatial,chellappa1993markov,moura1992recursive,balram1993noncausal,willsky2002multiresolution,vats2012finding}, see \cite{jordan2010major} for illustrative applications in several domains. A connection between GSP and graphical models can be seen in recent work on learning graph from data \cite{egilmez2017graph}, which makes use of Markov random field models to define optimality criteria for the learned graphs.  
%
\subsubsection{Historical perspective on graph signal processing}
\label{subsubsec:historiacalperspective}
%
We now briefly review some of the prior work that is more directly connected and in the spirit of signal processing on graphs, \cite{SandryhailaM:13,ShumanNFOV:13}. Although one can argue that any classification is arbitrary, we organize the discussion in two main streams of work. Some of these comments follow closely \cite{SandryhailaM:13,Sandryhaila2014big}.

\textbf{From algebraic signal processing (ASP) to graph signal processing (GSP).} The sequence of papers \cite{Pueschel:03a,Pueschel:05e,Pueschel:08a,Pueschel:08b,Pueschel:08c} introduced ASP, an axiomatic approach to time signal processing. ASP starts from a signal model~$\Omega$. Many signal models are possible, and a relevant question is to determine which one is more appropriate for a given application or should be associated with a given linear transform. One of the motivations to develop ASP was to answer a simple question: why is the discrete cosine transform~(DCT) the linear transform commonly associated with processing images leading, as experimentally observed, to better results in lossy image compression than the discrete Fourier transform~(DFT). The DCT (type~II) is associated with many of the lossy image/video compression standards \cite{sikora2005trends,lengwehasatit2004scalable}  from JPEG, to MPEG-1 \cite{le1992mpeg} 
%and MPEG-2 \cite{haskell1996digital} 
%video conference codecs like H.261, H.263, or 
to H.264/AVC \cite{hanzocherrimanstreit-08,luthra2003special} and HEVC. Based on~\cite{clarke1981relation}, see also item~6, page~153 in~\cite{jain1989fundamentals}, the energy compaction offered by the DCT was justified because the DCT asymptotically approximates the Karhunen-Lo\`eve transform (KLT) of a first order (causal) Markov process (a first order autoregressive AR(1) model). This of course is an unsatisfactory explanation since images are basically non-causal models with no left-right or up-down preferred direction; reference~\cite{Moura:98} does show more fittingly that the DCT and DST are the KLTs for first order \textit{non}-causal Markov random fields rather than causal Markov processes.  By appropriate definition of a \textit{space} signal model \cite{Pueschel:08b}, the DCT Type~II and each one of its other fifteen cousin trigonometric linear transforms are shown to be Fourier transforms playing, for the (corresponding) space model, the role that the DFT plays for the time (cyclic) model. References~\cite{Pueschel:03a,Pueschel:05e,Pueschel:08a,Pueschel:08b} show that, under appropriate conditions,  the signal model is generated from a simple filter, the \textit{shift}. In other words, under these conditions and signal model, choice of the shift determines filtering, convolution, the Fourier transform, frequency, and spectral analysis among other common concepts and constructs from traditional digital signal processing. This led \cite{SandryhailaM:13,Sandryhaila:2014ju} to introduce for signals indexed by nodes of an arbitrary directed or undirected graph the possibly weighted graph adjacency matrix as the shift that generates the graph signal model. This choice is satisfying in the sense that when the signal model is the time signal model or the  space signal model the shifts and the graph signal model revert to the shifts and signal models in~\cite{Pueschel:08a} and~\cite{Pueschel:08b}, respectively. Subsequently, authors have proposed other shifts obtained from the adjacency matrix of the signal graph assumed~\cite{giraultgoncalvesfleury-2015,gavilizhang-2017} that attempt to preserve isometry of the shift but lose the locality of the adjacency matrix shift.

\textbf{From graph Laplacian spectral clustering to Laplacian-based GSP.}
%
References \cite{Tenenbaum:00,Roweis:00,Belkin:03,Donoho:03} develop low-dimensional representations for large high-dimensional
data through spectral graph theory~\cite{Belkin:02,Belkin:03} and the graph Laplacian~\cite{Chung:96}, by projecting the data on a low-dimensional subspace generated by a small subset of the Laplacian eigenbasis. The use of the graph Laplacian is justified by assuming the data is smooth in the sense that if the dataset is large and samples uniformly randomly a low-dimensional manifold then the (empirical) graph Laplacian acting on a smooth function on this manifold is a good discrete approximation that converges pointwise and uniformly to the elliptic Laplace-Beltrami operator applied to this function as the number of points goes to infinity~\cite{heinaudibertluxburg-2005,ginekoltchinskii-2006,heinaudibertluxburg-2007}. References \cite{Coifman:05a,Coifman:05b,Coifman:06} choose discrete approximations to other continuous operators, for example, a conjugate to an elliptic Schr{\"o}dinger-type operator, and obtain other spectral bases for the characterization of the geometry of the manifold underlying the data.

In a different direction, motivated by processing of data collected by sensor networks where sensors are irregularly placed,   \cite{guestrinbodikthibauxpaskinmadden-ipsn2004} develops regression algorithms, \cite{ganesangreensteinestrinheidemanngovindan-2005,wagnerbaraniuketal-SSPWorkshop2005,wagnerbaraniuketal-IPSN06, Coifman:06,Hammond:11} wavelet decompositions,
\cite{Narang:10,Narang:12} filter banks on graphs, \cite{wagnerdelouillebaraniuk-2006} de-noising, and~\cite{Zhu:12} compression schemes using the graph Laplacian. Some of these references consider distributed processing of data from sensor fields, while others study localized processing of signals on graphs in multiresolution fashion by representing data using wavelet-like bases with varying ``smoothness'' or defining transforms based on node neighborhoods. For example \cite{Hammond:11} uses the graph Laplacian and its eigenbasis to define a spectrum and a Fourier transform of a signal on a graph. This definition of a Fourier transform was also proposed for use in uncertainty analysis on graphs~\cite{Agaskar:12a,Agaskar:12}. Besides using the graph Laplacian, these works apply to data indexed by undirected graphs with real, non-negative edge weights. This approach is more fully developed in~\cite{ShumanNFOV:13}, which  adopts the graph Laplacian as basic building block to develop GSP for data supported by undirected graphs.


